Exploring Real-Time Music-to-Image Systems for Creative Inspiration in Music Creation

This paper presents a study on the use of a real-time music-to-image system as a mechanism to support and inspire musicians during their creative process. The system takes MIDI messages from a keyboard as input which are then interpreted and analysed using state-of-the-art generative AI models. Based on the perceived emotion and music structure, the system's interpretation is converted into visual imagery that is presented in real-time to musicians. We conducted a user study in which musicians improvised and composed using the system. Our findings show that most musicians found the generated images were a novel mechanism when playing, evidencing the potential of music-to-image systems to inspire and enhance their creative process.

==> table1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[!ht]
\centering
\small
% \setlength{\tabcolsep}{1.2pt}
% \renewcommand{\arraystretch}{1.3}
\caption{The result of GPT-4 extracting musical features from input music ABC Notation using the prompt "What musical features can you extract from the following musical piece written in ABC Notation? \{\textit{Music in ABC Notation}\}"}\label{tab1}
\resizebox{1\linewidth}{!}{
\begin{tabular}{c|c}
\hline
Features                  & Answer                                                                                                                         \\ \hline
Instrument &
  \begin{tabular}[c]{@{}c@{}}The piece specifies two voices (V:1 and V:2) with the same program number (Program 1 0), \\ indicating they are both intended to be played on the piano. The second voice is labeled as "bass," \\ suggesting it plays a lower, supportive role in the harmonic texture.\end{tabular} \\ \hline
Time Signature            & The M:4/4 marking indicates a time signature of 4/4.                                                                           \\ \hline
Note Length               & The L:1/8 setting specifies that the default note length is an eighth note (quaver).                                           \\ \hline
Tempo                     & The Q:1/4=96 setting indicates a tempo of 96 quarter notes (crotchets) per minute.                                             \\ \hline
Key Signature             & The K:Em setting indicates the piece is in E minor.                                                                            \\ \hline
\multirow{2}{*}{Melody and Harmony} &
  \begin{tabular}[c]{@{}c@{}}The melody line in V:1 features a repetitive motif with variations in pitch, \\ primarily using longer note values (mostly dotted half notes followed by eighth notes), \\ which indicates a melodic theme that evolves gradually.\end{tabular} \\ \cline{2-2} 
 &
  \begin{tabular}[c]{@{}c@{}}The bass line in V:2 provides the harmonic foundation with a series of chordal patterns that repeat and evolve, \\ anchoring the piece in its E minor tonality. The use of brackets indicates chords played together, \\ with the progression moving through various harmonic intervals and contributing to the overall mood.\end{tabular} \\ \hline
Dynamics and Articulation & \begin{tabular}[c]{@{}c@{}}The use of ">" (accent) in V:1 suggests moments of emphasis or articulative interest,\\ particularly in shaping the melody line. \end{tabular} \\ \hline
Repetition and Variation &
  \begin{tabular}[c]{@{}c@{}}Both voices exhibit repetition and variation—a common compositional technique \\ to create cohesion and contrast. Voice 1 repeats a rhythmic pattern with slight melodic variations,\\  while Voice 2 repeats a harmonic pattern with changes that reflect the melodic alterations in Voice 1.\end{tabular} \\ \hline
\end{tabular}
}
\end{table*}

==> table2.tex <==
\begin{table*}[!ht]
\centering
%\small
\caption{The result of GPT-4 inferring emotion from musical features of input music ABC Notation using the prompt "What emotion can you infer from this musical piece written in ABC Notation? \{\textit{Music in ABC Notation}\}"}\label{tab2}
\resizebox{1\linewidth}{!}{
\begin{tabular}{c|c}
\hline
Features &
  Inference \\ \hline
Key Signature (E Minor) &
  \begin{tabular}[c]{@{}c@{}}The choice of E minor sets a somber or melancholic tone for the piece. \\ Minor keys are generally associated with sadness, introspection, or a contemplative mood.\end{tabular} \\ \hline
Tempo (96 BPM) &
  \begin{tabular}[c]{@{}c@{}}The moderate tempo of 96 beats per minute supports a reflective and somewhat introspective atmosphere. \\ It's just right for a contemplative or pensive mood.\end{tabular} \\ \hline
Melodic Repetition &
  \begin{tabular}[c]{@{}c@{}}The melody in the V:1 line features repeated phrases with slight variations. This repetition can create a sense of longing \\ or unresolved emotion, contributing to a reflective or melancholic atmosphere.\end{tabular} \\ \hline
Harmonic Support &
  \begin{tabular}[c]{@{}c@{}}The V:2 line provides a harmonic foundation that complements the melody. The chords and bass notes in the harmony\\  reinforce the key's emotional character, adding depth and richness to the piece's overall mood.\end{tabular} \\ \hline
Dynamic Contrast &
  \begin{tabular}[c]{@{}c@{}}The potential for dynamic contrast between the melody and harmony lines, and within the melodic line itself, \\ further emphasize the piece's emotional depth. The interplay between louder and softer passages \\ can enhance feelings of introspection or melancholy.\end{tabular} \\ \hline
\end{tabular}
}
\end{table*}

==> table3.tex <==
\begin{table*}[!ht]
\centering
\small
\setlength{\tabcolsep}{25pt}
\renewcommand{\arraystretch}{1.3}
\vspace{0.25cm}
\begin{tabular}{lll}
Musical piece & Genre     & Emotion Inferred by GPT-4           \\ \hline \hline
Rondo Alla Turca (Turkish March) - Mozart & Classical & Energetic, Lively, Complex          \\ 
Sonate No. 14, Moonlight 3rd Movement - Beethoven     & Classical & Vibrant, Intense, Energetic         \\
Clair de Lune - Debussy                   & Classcal  & Melancholic, Reflective, Serene     \\ 
Nocturne Op. 48 No.1 - Chopin             & Classical & Reflective, Tranquil, Introspective \\ 
The Piano Medley - Queen                  & Pop       & Dynamic, Bright, Whimsical          \\ 
Quantifiable connection - Interstellar    & Pop       & Urgent, Spirited, Exciting          \\ 
Feel My Pain - Jurrivh                    & Pop       & Meditative, Subdued, Somber         \\ 
La Storia - Alexander Descartes           & Pop       & Tranquil, Harmonious, Soothing      \\ 
Don't Jazz Me Rag - James Scott           & Jazz      & Joyful, Lively, Upbeat              \\ 
Suite Dansante en Jazz - Schulhoff        & Jazz      & Serene, Elegant, Graceful           \\ 
London Blues - Jelly Roll Morton          & Jazz      & Expressive, Uplifting, Bright       \\ 
\end{tabular}
\caption{The result of GPT-4 inferring emotion of different musical pieces using the prompt "What emotion can you infer from this musical piece written in ABC Notation? Answer this question using only three words. \{\textit{Music in ABC Notation}\}"}\label{tab3}
\end{table*}

==> table5.tex <==
\begin{table*}[]
\centering
%\small
\setlength{\tabcolsep}{4.3pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{c||cccc}
Participant ID & Age & Years of Music Experience & Years of Playing the Piano/keyboard & Years of Composition Experience \\ \hline \hline
P1 & 29 & Over 20 & 4       & 15          \\ 
P2 & 26 & Over 20 & Over 16 & 8           \\ 
P3 & 46 & Over 20 & Over 20 & Over 20     \\
P4 & 34 & Over 20 & Over 20 & 18          \\ 
P5 & 30 & Over 20 & 3-5     & Less than 1 \\ 
\end{tabular}
\caption{The demographic information and music proficiency of 5 participants.}\label{tab5}
\end{table*}
